Clifford algebra and the projective model of Elliptic spaces

I apply the algebraic framework developed in arXiv:1101.4542 to study geometry of elliptic spaces in 1, 2, and 3 dimensions. The background material on projectivised Clifford algebras and their application to Cayley-Klein geometries is described in arXiv:1307.2917. The use of Clifford algebra largely obviates the need for spherical trigonometry as elementary geometric transformations such as projections, rejections, reflections, and rotations can be accomplished with geometric multiplication. Furthermore, the same transformations can be used in 3-dimensional elliptic space where effective use of spherical trigonometry is problematic. I give explicit construction of Clifford parallels and discuss their properties in detail. Clifford translations are represented in a uniform fashion by geometric multiplication as well. The emphasis of the exposition is on geometric structures and computation rather than proofs.

==> g-1.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.887807,113.958449)(-0.500000,-1.000000){$w$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.107512,229.676408)(-1.000000,-0.500000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-85.376640,221.199366)(0.000000,-0.360142){$E_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-85.376640,173.320193)(0.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-106.621304,121.871967)(0.000000,-0.500000){$\alpha$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-85.376640,144.989321)(0.000000,-0.500000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-96.730623,124.249479)(0.000000,-0.281250){$\beta$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-65.127949,187.802671)(-0.138996,0.215858){$r_{ab}$}


==> g-10+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-10+0_0.pdf}%
}%


==> g-10.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-10+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751624274,3Droll=0,3Droo=410.889700647751624274,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-10+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-10+0.prc}}


==> g-11+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-11+0_0.pdf}%
}%


==> g-11.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-11+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751624274,3Droll=0,3Droo=410.889700647751624274,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-11+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-11+0.prc}}


==> g-12+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-12+0_0.pdf}%
}%


==> g-12.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-12+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751624274,3Droll=0,3Droo=410.889700647751624274,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-12+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-12+0.prc}}


==> g-13+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-13+0_0.pdf}%
}%


==> g-13.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-13+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858114178602,3Droll=0,3Droo=409.971468858114178602,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-13+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-13+0.prc}}


==> g-14+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-14+0_0.pdf}%
}%


==> g-14.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 223.227250pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,111.613625)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-14+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -403.803958610462245815,3Droll=0,3Droo=403.803958610462245815,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-14+0.js]{254.9525pt}{220.825pt}{\ASYprefix\jobname-14+0.prc}}


==> g-15+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-15+0_0.pdf}%
}%


==> g-15.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-15+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.847616332356096791,3Droll=0,3Droo=410.847616332356096791,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-15+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-15+0.prc}}


==> g-16+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-16+0_0.pdf}%
}%


==> g-16.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-16+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.847616332356096791,3Droll=0,3Droo=410.847616332356096791,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-16+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-16+0.prc}}


==> g-17+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-17+0_0.pdf}%
}%


==> g-17.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-17+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.847616332356096791,3Droll=0,3Droo=410.847616332356096791,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-17+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-17+0.prc}}


==> g-18+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-18+0_0.pdf}%
}%


==> g-18.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-18+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -421.43382632336243887,3Droll=0,3Droo=421.43382632336243887,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-18+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-18+0.prc}}


==> g-19+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-19+0_0.pdf}%
}%


==> g-19.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 223.227250pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,111.613625)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-19+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -403.803958610462245815,3Droll=0,3Droo=403.803958610462245815,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-19+0.js]{254.9525pt}{220.825pt}{\ASYprefix\jobname-19+0.prc}}


==> g-2.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-2_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.887807,113.958449)(-0.500000,-1.000000){$w$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.107512,229.676408)(-1.000000,-0.500000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-85.376640,221.199366)(0.000000,-0.360142){$E_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-85.376640,173.320193)(0.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-106.621304,121.871967)(0.000000,-0.500000){$\alpha$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-85.376640,31.665834)(0.000000,-0.500000){$\textbf{c}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-105.863429,110.031993)(0.000000,-0.500000){$\kappa$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-111.168247,163.900645)(0.000000,0.205126){$r_{ac}$}


==> g-20+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-20+0_0.pdf}%
}%


==> g-20.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-20+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -409.971468858114008071,3Droll=0,3Droo=409.971468858114008071,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-20+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-20+0.prc}}


==> g-21+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-21+0_0.pdf}%
}%


==> g-21.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-21+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -416.64103882626199038,3Droll=0,3Droo=416.64103882626199038,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-21+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-21+0.prc}}


==> g-22+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-22+0_0.pdf}%
}%


==> g-22.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-22+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.847616332356210478,3Droll=0,3Droo=410.847616332356210478,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-22+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-22+0.prc}}


==> g-23+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-23+0_0.pdf}%
}%


==> g-23.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 238.283510pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,119.141755)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-23+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -453.649899005012116504,3Droll=0,3Droo=453.649899005012116504,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-23+0.js]{254.9525pt}{235.88125pt}{\ASYprefix\jobname-23+0.prc}}


==> g-3+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-3+0_0.pdf}%
}%


==> g-3.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-3+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751283213,3Droll=0,3Droo=410.889700647751283213,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-3+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-3+0.prc}}


==> g-4+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-4+0_0.pdf}%
}%


==> g-4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-4+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -410.889700647751453744,3Droll=0,3Droo=410.889700647751453744,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-4+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-4+0.prc}}


==> g-5+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-5+0_0.pdf}%
}%


==> g-5.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-5+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751737961,3Droll=0,3Droo=410.889700647751737961,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-5+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-5+0.prc}}


==> g-6.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-6_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-149.773521,111.931838)(-1.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-173.440204,140.323521)(-0.500000,-0.779180){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-134.170600,155.464362)(0.000000,-1.000000){$\textbf{R}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-148.905366,128.693796)(-0.660105,0.000000){$\alpha$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-185.821685,147.587133)(-1.000000,-0.179161){$\beta$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-147.794368,167.169322)(-1.000000,0.214051){$\gamma$}


==> g-7+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-7+0_0.pdf}%
}%


==> g-7.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-7+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 0.999999999999999889,3Dcoo=0 0 -410.889700647751453744,3Droll=0,3Droo=410.889700647751453744,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-7+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-7+0.prc}}


==> g-8.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-8_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073582,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-36.206789,83.540155)(-1.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-173.440204,149.773521)(-0.500000,0.220820){$\textbf{Q}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-137.950600,162.788112)(-0.500000,0.000000){$\textbf{R}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-9.049386,69.644884)(-0.750000,-1.000000){$\alpha$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-173.440204,135.250600)(-0.500000,-0.781250){$\beta$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-138.962267,149.498248)(-0.551458,-0.688888){$\gamma$}


==> g-9+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-9+0_0.pdf}%
}%


==> g-9.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-9+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751624274,3Droll=0,3Droo=410.889700647751624274,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-9+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-9+0.prc}}

